Evaluating Code Generation of LLMs in Advanced Computer Science Problems

Large Language Models (LLMs), such as GitHub Copilot and ChatGPT have become popular among programming students. Students use LLMs to assist them in programming courses, including generating source code. Previous work has evaluated the ability of LLMs in solving introductory-course programming assignments. The results have shown that LLMs are highly effective in generating code for introductory Computer Science (CS) courses. However, there is a gap in research on evaluating LLMs' ability to generate code that solves advanced programming assignments. In this work, we evaluate the ability of four LLM tools to solve programming assignments from advanced CS courses in three popular programming languages, Java, Python, and C. We manually select 12 problems, three problems from introductory courses as the baseline and nine programming assignments from second- and third-year CS courses. To evaluate the LLM-generated code, we generate a test suite of 1000 test cases per problem and analyze the program output. Our evaluation shows that although LLMs are highly effective in generating source code for introductory programming courses, solving advanced programming assignments is more challenging. Nonetheless, in many cases, LLMs identify the base problem and provide partial solutions that may be useful to CS students. Furthermore, our results may provide useful guidance for teachers of advanced programming courses on how to design programming assignments.

==> sections/conclusions___future_work.tex <==

\section{Conclusion}
% Our results indicate that although ACG tools are highly capable of deciphering complex problem descriptions, their effectiveness is negatively correlated to the description complexity.

In this paper, we investigate the capabilities of \ac{LLM} tools to
solve advanced programming assignments.
%
Our results indicate that compared to introductory course assignments,
\ac{LLM} tools struggle to generate correct source code for advanced
assignments.
%
However, the tools are often able to recognize the algorithm needed to
solve the assignment.
%
Our analysis on partially correct results shows that \acp{LLM} have
difficulty adjusting known algorithms to specific constraints and
often tend to implement popular heuristics instead of following the
prompt instructions.
%
We believe that teachers may use these insights to assess the knowledge
of students in advanced \ac{CS} courses by incorporating variations or constraints to known algorithms in advanced programming assignments.




==> sections/selected-problems.tex <==

\section{Selected Problems}
\label{chap:problems}

Each of the following sections includes a description of a selected problem and the problem prompt.

\subsection{Temperature Measurements}
\label{chap:temp-problem}
This problem is a variant of the Rainfall problem~\cite{soloway1986learning} and was given as the first assignment in a university-level introductory programming course. The assignment consists of reading a set of temperature measurements for a given amount of weeks, and then calculating the minimum, maximum, and average temperature, both for all the individual weeks and the entire period as a whole. 
The prompt for the problem is this following:


\subsection{Sorting People}
\label{chap:sorting}
Sorting elements in a list into a specified order is a fundamental skill in programming, which is the reason for manually designing this problem. Given a list, consisting of a set of people, each with their respective assigned attributes, name, height, weight, age and hometown, the problem is to sort the people in ascending order with the following priority: 
\begin{inparaenum}
    \item Height
    \item Weight
    \item Age
    \item Hometown
    \item Name.
\end{inparaenum}
%
The prompt for this problem is the following:

\subsection{Box Problem}
\label{chap:boxes}
This problem was taken from a lecture in a second cycle CS course. It is a rephrased NP-hard packing problem~\cite[Chapter~8]{kleinberg_tardos}. The problem was chosen due to its straightforward description. There exist many variations to this problem, and the selected variation uses only positive integers to keep the description simple. 

The problem consists of packing items with different weights into boxes with a set weight capacity. There exists an infinite number of boxes, and the problem is to utilize the capacity of the boxes such that every box fits as many items as possible.
%
The prompt for this problem is the following:

\subsection{Traveling Salesman Problem}
\label{sec:tsp}
The \ac{TSP}~\cite[Chapter~2]{kleinberg_tardos} is a famous problem within computer science. Depending on the formulation, it is either an optimization problem or a decision problem. The problem is an NP-hard problem. A  concise description of the problem is given by \citeauthor{garey1979computers}~\cite{garey1979computers}: ``Given a set of cities $c_1, c_2 ... c_i$ and distances between each pair, noted as $d_1, d_2 ... d_j$. How should the salesman travel, such that he visits every city once and travels the shortest possible distance?''. 


Due to the problem being well known, we rephrased the problem as a teacher who wants to hand out tests to students in a class. The students are sitting at different distances between each other, and the teacher wants to visit every student once, while traveling the shortest distance.
%
The prompt for this problem is the following:

\subsection{Electrical Outlets Problem}
\label{chap:outlets}
This problem was used to examine the ability to construct efficient algorithms in a second cycle university course on algorithms, data structures and complexity, during Fall 2022.

There were three main reasons to include this problem in our evaluation. Firstly, this problem is a rephrasing of the known graph problem minimum spanning tree~\cite[Chapter~4]{kleinberg_tardos}, an important concept in \ac{CS}.
%
Secondly, it contains an element of finding the optimal solution without being an NP-complete problem.
Lastly, the problem description is unclear and possibly not available in the training set of the \acp{ACG}. 

The prompt for this problem is the following:

\begin{promptbox}{Traveling}
  Unfortunately, it often happens that the last flight (Xn-1 Xn) of each destination is overbooked. In these cases, the company reserves the right to change (at departure) the flights of its customers with final destination Xn to another route, but to not disappoint them too much, it always changes the route to the one with the next minimum total travel duration.
\end{promptbox}


